Towards Learning Universal Hyperparameter Optimizers with Transformers

Meta-learning hyperparameter optimization (HPO) algorithms from prior experiments is a promising approach to improve optimization efficiency over objective functions from a similar distribution. However, existing methods are restricted to learning from experiments sharing the same set of hyperparameters. In this paper, we introduce the OptFormer, the first text-based Transformer HPO framework that provides a universal end-to-end interface for jointly learning policy and function prediction when trained on vast tuning data from the wild, such as Google's Vizier database, one of the world's largest HPO datasets. Our extensive experiments demonstrate that the OptFormer can simultaneously imitate at least 7 different HPO algorithms, which can be further improved via its function uncertainty estimates. Compared to a Gaussian Process, the OptFormer also learns a robust prior distribution for hyperparameter response functions, and can thereby provide more accurate and better calibrated predictions. This work paves the path to future extensions for training a Transformer-based model as a general HPO optimizer.

==> storage/abstract1.tex <==
%In this paper, we investigate the following question: 
To what extent can a Transformer be used to learn custom function priors and algorithms from offline blackbox and hyperparameter optimization data? We discover that from purely token-based representations, Transformers are capable of learning to jointly predict parameter and function values from complex objectives and algorithms, respectively leading to the construction of flexible token-based blackbox optimizers and accurate function regressors. In particular, the Transformer can simultaneously and precisely imitate the behavior of at least 7 different algorithms, which can be further improved via its function uncertainty estimates, at times significantly more accurate than Gaussian Processes. Furthermore, through numerous ablation studies, we find that these trained models are strong meta-learners, capable of utilizing various textual metadata to assist in prediction. Our work is the first framework to apply optimization over textual representations over various search spaces, and suggests that Transformers may be a universal interface for learning complex tuning data from the wild.


==> storage/data.tex <==
For practical purposes, we consider a purely offline training approach and obtain three training datasets $\mathcal{D}$ from two sources (described in more detail in \cref{appendix:data}): 
\begin{enumerate}[leftmargin=*]
\item Offline HPO studies collected in the past by any standard HPO algorithms. We use a large collection of about 750K proprietary hyperparameter tuning studies, denoted as \textbf{\vizierdata}, each with on average 300 trials\footnote{Anonymized due to the blind review requirement.}, covering a vast class of machine learning models with applications from vision, speech, to NLP and robotics and represents a distribution of HPO tasks in practice. All studies include metadata and hyperparameters to different extents.
\item Generated studies from running standard HPO algorithms on surrogate functions from black-box optimization and HPO benchmarks \textbf{\bbobdata} \citep{ElHara2019COCOTL} and \textbf{\hpobdata} (continuous) \citep{hpo-b}. \bbobdata consists of a collection of 24 types of synthetic functions with customizable properties (dimension sizes, rotations, shifts, discretizations, noise types) we randomize over, while \hpobdata contains the largest public benchmark of datasets for HPO over 6M evaluations over 16 test search spaces, over a wide range of ML-based models.
\end{enumerate}

While all datasets' algorithms use a mixture of non-adaptive, evolutionary, and BO algorithms, these algorithms' behaviors may change over time in \vizierdata, and thus the corresponding $A_{b}$ must be treated as a nonstationary mixture of algorithms, whose algorithm name field in $m$ is therefore set to empty.
To still have at least one controlled baseline, we include the trust-region based BO baseline using a GP-UCB acquisition function from \cite{vizier}, which we term "Vizier GP-UCB".

%GP-UCB is a classical Bayesian optimization method that heavily relies on observations and probabilistic modeling to generate the next parameters. 

In contrast, for \bbobdata and \hpobdata, we may precisely control the algorithms used, which are: (1) Grid Search, (2) Shuffled Grid Search, (3) Random Search, (4) Regularized Evolution \cite{real2019regularized}, (5) Hill-Climbing, (6) Eagle Strategy \cite{yang2010eagle}, and (7) GP-UCB \cite{rasmussen2003gaussian}. In these cases we include the algorithm name in $m$ as part of the conditioning input for our model. We summarize these differences in \cref{table:dataset_differences}.

\begin{table}[h]
\begin{center}
\begin{tabular}{ |c|c|c|c| } 
 \hline
  & \textbf{\vizierdata} & \textbf{\bbobdata} & \textbf{\hpobdata} \\
  \hline \hline
 Source Type & Source 1 & Source 2 & Source 2 \\ 
 \hline
 $A_{b}$ & Non-stationary & Controlled & Controlled \\
 \hline
 Objective Functions & HPO tasks & Synthetic & HPO tasks \\
 \hline
Search space & Different per task & Randomized & 16 shared continuous spaces \\
 \hline
 $m$ metadata & User-Dependent & Algo. name & Algo. \& Parameter Name \\
 \hline
 Test Function & GP Surrogate & Actual Functions & Random Forest Surrogate \\
 \hline
\end{tabular}
\end{center}
\caption{Comparison of the offline datasets.}
\label{table:dataset_differences}
\end{table}


==> storage/data_setup.tex <==

We consider three training datasets from the two sources described in \cref{sec:dataset}, with more details outlined in \cref{appendix:data}.

For Source 1, we have access to a large collection of proprietary machine learning hyperparameter tuning studies, denoted as \textbf{\vizierdata}\footnote{Details omitted due to the blind review requirement.}. It covers a vast class of models with applications from vision, speech, to NLP and robotics. All studies include metadata and hyperparameters to different extents, and are generated by different types of HPO algorithms (whose behaviors may change over time), such as GP-based BO, random search, evolution algorithms. \vizierdata represents a distribution of HPO tasks in practice. We split the dataset in temporal order to avoid information leak, use $\sim$500K studies for training, and select 16 studies generated by a different set of users for testing. Because the dataset does not record the algorithm's implementation which generated a given study, we must treat the behavior policy $A_b$ as a stochastic mixture of algorithms, and leave the algorithm name in the metadata $m$ empty. For each test function, we fit a GP as a surrogate function for optimization.

For Source 2, we consider two large-scale black-box optimization benchmarks: \textbf{\bbobdata}
\citep{ElHara2019COCOTL} and \textbf{\hpobdata} \citep{hpo-b}. In summary, \bbobdata consists of a collection of 27 customizable synthetic functions whose properties (dimension sizes, rotations, shifts, discretizations, noise types) we significantly randomize over, while \hpobdata contains the largest public benchmark of datasets for HPO over 6.4M evaluations over 176 search spaces, over a wide range of ML-based models. For each of the two benchmarks, we generate an offline dataset by applying a collection of the following algorithms: (1) Grid Search, (2) Shuffled Grid Search, (3) Random Search, (4) Regularized Evolution \cite{real2019regularized}, (5) Batch Hill-Climbing \cite{golovin2019gradientless} (6) Eagle Strategy \cite{yang2010eagle} (7) Gaussian Process (GP-UCB) \cite{rasmussen2003gaussian}. The first three algorithms are non-adaptive search algorithms whose behavior does not depend on the observed values, while the middle three (Regularized Evolution, Hill Climbing, Eagle Strategy) are evolutionary algorithms that should bias the trajectory into promising regions. GP-UCB is a classical Bayesian optimization method that heavily relies on observations and probabilistic modeling to generate the next parameters. For Source 2, since we know the choice of algorithm that generated a given trajectory, we include the algorithm name in $m$ as part of the conditioning input for our model.

We include all the algorithms mentioned above as baselines where appropriate. Additionally, in the \vizierdata test set, we include a standard BO baseline with GP-UCB acquisition function. In the \hpobdata test set, we include the GP and DGP (GP with deep kernel) baselines provided by \citet{hpo-b} and a transfer-learning BO method. \footnote{Please note that none of the prior transfer-learning HPO methods can be applied across different search spaces as in the \vizierdata test set.}

We train a Transformer model with 250M parameters for each of the three datasets, \bbobdata, \vizierdata, \hpobdata, denote each trained model with a corresponding suffix of "-B", "-P", and "-H" respectively, and evaluate mainly on the test sets of the two natural HPO datasets \vizierdata and \hpobdata. Details of hyper-parameters are given in \cref{sec:training_details}. We will also investigate the effect of different domain gaps in transfer learning, that is from a blackbox benchmark domain to HPO "B$\rightarrow$ P/H", from a diverse HPO domain to more specific domain "P$\rightarrow$ H", and in domain "P/H$\rightarrow$ P/H".
% For \bbobdata, as all parameters are named as "xi" with $i\in[0,D)$ and always have value range in $[-5,5]$, significantly different from the other two datasets, we omit their parameter names and value in the metadata $m$ and only keep parameter type information.

In order to aggregate results across functions of different output scaling, we convert every tuning task to a maximization problem (via flipping the sign for minimization tasks), and define our performance metric at trial count $t$ as the best-so-far normalized function value, i.e. $\max_{i\in\{1:t\}} (y_{i} - y_\mathrm{rand})/(y_\mathrm{max} - y_\mathrm{rand})$. $y_\mathrm{rand}$ is defined as the median of function values randomly sampled in the search space to be robust to some function with extreme outliers, and $y_\mathrm{max}$ the maximum if known, or best value found by any algorithm. For \hpobdata, we use the bounds provided by the paper.

==> storage/dataset_and_model_training.tex <==

\section{Dataset and Model Training}

\subsection{Training Datasets}\label{sec:dataset}
Ideally, we would like to train our Transformer model as a policy in the same family of hyperparameter response functions as the test scenario and generate new optimization trajectories for training after every parameter update in an online fashion. However, it is usually not feasible or too expensive to create new trajectories online because generating a new trial means training a new model on some dataset. Even if cheap surrogate functions are available during training, repeatedly running Transformers to generate optimization trajectories could still be too expensive.

Therefore, in this work, we consider a pure offline training approach and obtain the training dataset, $\mathcal{D} = \{\tau_{i} | i \ge 0 \}$, from two sources: \textbf{(1)} offline HPO studies collected in the past by any standard HPO algorithms, and \textbf{(2)} running standard HPO algorithms on cheap surrogate functions to generate a single large set of studies. The surrogate function $f$ could be sampled from a family $\mathcal{F}$ of synthetic functions, and be a regression model fitted to a set of real experiment trials. Similarly, the algorithm $A$ to generate the trajectories can be sampled from a family $\mathcal{A}$ of common optimizers.

%While it is possible to train a model online with surrogate functions from source 2, doing so requires a significantly larger amount of computation to generate a vast amount of studies for every training instance when one may have to test various training hyper-parameters. Also, deploying a large sequence model to generate training data is inefficient and would require a large amount of GPUs as parallel data producer.

Using the terminology of offline reinforcement learning, the algorithm to generate the offline dataset is called the behavior policy $A_b$. It could refer to a single policy or a mixed policies with a random distribution over the set of base policies $\{A_a\}$, with $A_b = A_a, a\sim \mathrm{Uniform}\{a\}$.

\subsection{Model Training}

We train the Transformer model on the offline dataset to predict the next token autoregressively
%as a supervised learning problem by minimizing a weighted cross entropy of the output distribution sequence with the target optimization history sequence $\widehat{h}$
% \begin{equation}
%     \ell(\theta)
%     = \sum_n w_n \mathrm{CrossEnt}(D_{\theta_D}(E_{\theta_E}(\widehat{m})), \widehat{h}[1:n-1]), \widehat{h}[n]), \text{ with $w_n = 0$ if $\widehat{h}_n \in \{s_p, s_t\}$, otherwise 1}
% \end{equation}
\begin{equation}
    \mathcal{L}(\theta)
    = \sum_n w_n \log P_{\theta}(\widehat{h}[n]|\widehat{m}, \widehat{h}[1:n-1]), \text{ with $w_n = 0$ if $\widehat{h}_n \in \{s_p, s_t\}$, otherwise 1}
\end{equation}
We mask out the prediction of separator tokens in the loss and only predict parameter tokens, that is, to predict the action taken by the behavior policy $A_\mathrm{prior}$, also known as behavior cloning. We also include the loss for predicting function value tokens as an auxiliary task as we find it does not hurt the accuracy of parameter prediction and we get a probabilistic model for $p(y_t|\vx_t, \{\vx_i,y_i\}_{i=1}^{t-1})$.

We also include two types of data augmentation to mitigate overfitting to the training dataset. (1) As serializing the study imposes an unwanted order of parameters in the token sequence, we randomly permute the order of parameters for every study. The random order is kept consistent among the metadata $\widehat{m}$ and every serialized trial $\widehat{\vx}_t$. This allows the Transformer to learn to make predictions invariant to parameter order but can still look up the parameter configuration from metadata according to its order in each trial. (2) We normalize the function value $y_t$ in our data serialization step with the minimum and maximum value, $[y_\mathrm{min}, y_\mathrm{max}]$, in an existing study. But when applying the Transformer policy to optimize a new function, we usually do not have the knowledge about the range. In order for the Transformer to be robust to different normalization range, we apply a random scaling and shifting to the normalized function value before quantization in \cref{eq:quantization},
\begin{equation}
    y_\mathrm{norm} = (y - y_\mathrm{min})/(y_\mathrm{max} - y_\mathrm{min}) * s + c, s \sim \mathrm{Uniform}[0.3, 1], c \sim \mathrm{Uniform}[0, 1-s]
\end{equation}
The range of normalized $y$ will be $[c, c+s] \subseteq[0, 1]$ after transformation.


==> storage/inference.tex <==

\subsection{Data postprocessing and inference}
\label{appendix:inference}

\paragraph{Parameter prediction:} In the tokenized space, we now may predict $P_{\theta}(\widehat{x}_t^{(d)}|\widehat{m}, \widehat{h}_{t}^{(d-1)})$. To convert the parameter token $\widehat{x}_t^{(d)}$ back into an actual parameter value $x_t^{(d)}$, we truncate the discrete output distribution to the subset of vocabulary with valid parameter values:
\begin{equation}
    p_\theta(x_t^{(d)}|m, h_{t}^{(d-1)}) = \mathcal{PW}(x_t^{(d)}; P_\theta(\widehat{x}_t^{(d)}|\widehat{m}, \widehat{h}_{t}^{(d-1)}), \mathcal{X}^{(d)})\,,
\end{equation}
where $\mathcal{PW}(\cdot; P, \mathcal{X})$ denotes a piece-wise constant distribution mapped from the discrete distribution $P$ to the original domain $\mathcal{X}$. Specifically, for a \texttt{Double} parameter $x$ with range $\left[x_\mathrm{min}, x_\mathrm{max}\right]$ and quantization level $Q$, $\mathcal{PW}(x; P, x_\mathrm{min}, x_\mathrm{max}) = P(\widehat{x}) / (x_\mathrm{max} - x_\mathrm{min}) * Q$, and for all the other parameter types, $\mathcal{PW}(x; P, \mathcal{X}) = P(\widehat{x})$.

Consequently, we could define an HPO policy by sampling parameter values from the prior defined by the Transformer as follows:
\begin{equation}
    A_{\text{Prior}}(\vx_t|m, h_{t-1}) = \prod_{d=1}^D p_\theta(x_t^{(d)}|m, h_{t}^{(d-1)}),
    \text{ where } h_{t}^{(d-1)} = h_{t-1}, x_{t,1}, \cdots, x_{t,d-1}
\end{equation}
As we use a supervised learning loss, we expect $A_{\text{Prior}}$ approximates the behavior policy $A_b$.

\paragraph{Function prediction:} We may also now predict $P_{\theta}(\widehat{y}_t|\widehat{m}, \widehat{h}_{t}^{(D)})$ in the token space. To convert the function token $\widehat{y}_t$ back to a floating point value $y_t$, we define a piecewise constant distribution similarly to the \texttt{Double} parameter:
\begin{equation}
    p_\theta(y_t|m, h_{t-1}, \vx_t) = \mathcal{PW}(y; P_\theta(\widehat{y}_t|\widehat{m}, \widehat{h}_{t}^{(D)}), y_\mathrm{min}, y_\mathrm{max})
\end{equation}
Note that the predicted distribution of $y$ is limited to to range of $[y_\mathrm{min}, y_\mathrm{max}]$. This is not a concern for HPO when either the range is known or we set the range large enough compared to observed values. For more general use as a few-shot function prediction model, one could consider adopting the Riemann Distribution in \cite{gp_transformer}, which supports an unbounded range.

\paragraph{Augmented HPO policies with function prediction:} In the behavioral cloning setting, at best, the learned policy $A_{\text{Prior}}$ can only perform as well as the original policy $A_{b}$. However, we can take advantage of the model's simultaneous function prediction ability to improve the policy with model-based planning or offline reinforcement learning techniques. While a comprehensive study of policy improvement for Transformers is out of the scope of this work, here we consider a simple policy improvement operator: sampling $M$ candidate suggestions from $A_{\text{Prior}}$ and choosing the suggestion with the highest score defined by an acquisition function $u$ as follows:
\begin{equation}
    A_{u}(\vx_t|m, h_{t-1}) = \underset{\{\vx^i\}_{i=1}^M}{\mathrm{argmax}} ~ u(p_\theta(\cdot|m, h_t, \vx^i)), \text{ with } \vx^i \sim A_{\text{Prior}}(\vx|m, h_{t-1}), \forall i
\end{equation}
Common acquisition functions include Upper Confidence Bound (UCB), expected improvement (EI), and Thompson Sampling (TS). Moreover, we can extend Thompson sampling to multiple steps, $n\geq 1$, thanks to the efficiency of sampling one history by a single forward-pass to the model:
\begin{equation}
    u_{TS(n)}(\vx) = \max\{y_{t'}\}_{t'=t}^{t+n-1} , \text{ with } \vx_{t}=\vx, y_{t'} \sim p_\theta(\cdot|m, h_{t'}, \vx_{t'}), \vx_{t'+1} \sim A_{\text{Prior}}(\vx|m, h_{t'}), \forall t'
\end{equation}
At a high level, this approach to combining imitated policies with function prediction is reminiscent of the idea of Batch-Constrainted Deep Q-Learning (BCQ) \citep{fujimoto2019off}.


==> storage/intro1.tex <==
Over the past few years, Transformers \citep{Transformer} have dramatically risen in popularity as a universal model for understanding a multitude of different data types, ranging from natural language \citep{bert}, images \citep{vision_Transformer, image_gpt}, biological data \citep{bio_Transformer, bio_Transformer2}, and code \citep{alphacode, codex}.

With the rise of hyperparameter optimization services such as Vizier \cite{vizier} which can store large amounts of tuning data, an increasingly abundant data type are blackbox and hyperparameter optimization trajectories, which can hold key information about the structure of users' objectives and the algorithms used to tune these objectives. In fact, recently benchmarks such as \citep{hpo-b, dnn_bench} have been proposed, which indeed contain such tuning data. Given sufficient offline data, one may potentially meta-learn both a better prior distribution over the set of possible blackbox functions to be tuned, as well as a better optimization algorithm directly. 

However, dealing with a large dataset of tuning experiments in the wild can be a challenging task, requiring a model to support a flexible input space with mixed text and numerical values due to the extensive variability in the objective's search space definition and potential textual metadata. As the Transformer has been shown to be the de-facto model for learning over massive amounts of data over flexible token-based spaces, a natural question to ask is whether it is capable of meta-learning from very large amounts of numerical optimization data.

In this paper, we seek to answer this question, and our core contributions are the following:
\begin{itemize}
\item In order to process complex tuning data at scale, we provide a novel tokenization framework, whose particular design choices, especially for dealing with the scaling of numerical data, greatly reduce required sequence lengths for autoregressive models without loss of information.
\item We discover that over purely token-based representations, Transformers are capable of simultaneously learning the behaviors of at least 7 diverse blackbox optimization algorithms from broad classes of methods (non-adaptive, evolutionary, and Bayesian), and replicating said algorithms over unseen search spaces and objective functions in a zero-shot manner.
\item Furthermore, Transformers are able to learn an inherent prior over objective functions and thus predict function outputs accurately, and in many cases significantly surpass Gaussian Processes in standard metrics such as negative log-likelihood (NLL) and expected confidence error (ECE). Such predictions may be used to augment and improve the Transformer's own HPO policies in a Bayesian Optimization-like fashion.
\item Through comprehensive ablation studies in the Appendix, we discover that the Transformer is capable of utilizing textual metadata (such as function names) to improve its predictions, thus acting as a very flexible and adaptive meta-learner.
\end{itemize}

==> storage/intro_list.tex <==

\begin{comment}
\begin{enumerate}
    \item Hyperparameter optimization includes various sources of information including experiment meta-information, parameter information.
    \item Traditional Bayesian-optimization treats hyper-parameter optimization as black-box optimization and ignores a lot of information.
    \item One may learn a better prior information about the model to optimize by taking advantage of as much information in the data as possible
    \item To achieve that, an optimizer needs to deal with various semi-structure data, e.g. textual information, various parameter types, values, and dependencies.
    \item We propose a flexible framework to learn hyperparameter optimizers with a universal interface to learn from tuning experiment datasets based on Transformer.
    \item By learning on a wild range of tuning experiments, we show
    \begin{enumerate}
        \item The optimizer can learn variable type of algorithms.
        \item The optimizer learns an inherent probabilistic model of functions.
        \item The optimizer achieves a comparable performance with strong baselines without further adaptation on experiments of the same search space.
    \end{enumerate}
    \item This framework provides numerous extensions for future research.
\end{enumerate}
\end{comment}


==> storage/model1.tex <==

With the serialized and tokenized study, we are ready to model the distribution of $\tau$ with a sequence model, such as a Transformer. Denote the tokenized integer sequence of any data $a$ as $\widehat{a} \in \{0, \dots, V-1\}^{|\widehat{a}|}$ where $V$ is the size of the vocabulary. In this work, because we convert every quantized number in $h$ to a single token, we have $\widehat{x}_t^{(d)}=q(x_{t}^{(d)})$, $\widehat{y}_t^{(d)}=q(y_{t}), \forall t,d$. We also denote the two constant separator tokens between parameters \texttt{"*"} as $s_p$, and between two trials \texttt{"|"} as $s_t$. These tokens are used to inform a sequence model the parameter dimension and metric dimension. The joint distribution of the optimization history $h$ conditioned on metadata $m$ can be written using the chain rule as
% \begin{align}
%     &P(\widehat{h}|\widehat{m}) 
%     = P\left(\widehat{x}_1^{(1)}, \widehat{x}_1^{(2)}, \dots, \widehat{x}_1^{(D)}, s_p, \widehat{y}_1, s_t, \dots,
%           \widehat{x}_T^{(1)}, \widehat{x}_T^{(2)}, \dots, \widehat{x}_T^{(D)}, s_p, \widehat{y}_T | \widehat{m} \right) \nonumber\\
%     &= \prod_{t=1}^T \left(\prod_{d=1}^D P(\widehat{x}_t^{(d)}|\widehat{m}, \widehat{h}_{1:n(\widehat{x}_t^{(d-1)})})\right) 
%                      P(s_p|\widehat{m}, \widehat{h}_{1:n(s_p)-1})
%                      P(\widehat{y}_t|\widehat{m}, \widehat{h}_{1:n(\widehat{y}_t)-1})
%                      P(s_t|\widehat{m}, \widehat{h}_{1:n(s_t)-1})\,,
% \end{align}
\begin{align}
    &P(\widehat{h}|\widehat{m}) 
    = P\left(\widehat{x}_1^{(1)}, \widehat{x}_1^{(2)}, \dots, \widehat{x}_1^{(D)}, s_p, \widehat{y}_1, s_t, \dots,
          \widehat{x}_T^{(1)}, \widehat{x}_T^{(2)}, \dots, \widehat{x}_T^{(D)}, s_p, \widehat{y}_T | \widehat{m} \right) \nonumber\\
    &= \prod_{t=1}^T \left(\prod_{d=1}^D P\left(\widehat{x}_t^{(d)}|\widehat{m}, \widehat{h}_{t}^{(d-1)}\right)\right) 
                     P\left(s_p|\widehat{m}, \widehat{h}_{t}^{(D)}\right)
                     P\left(\widehat{y}_t|\widehat{m}, \widehat{h}_{t}^{(D)}\right)
                     P\left(s_t|\widehat{m}, \widehat{h}_t\right)
\end{align}

%where $D$ is the number of parameters in the given study and $\widehat{h}_{t,\cdot}$ denotes the optimization history before the corresponding token in trial $t$.
% where $D$ is the number of parameters in the given study and $n(\cdot)$ denotes the index of a token in the optimization history sequence.

Predicting the constant separator tokens $s_p$ and $s_t$ is trivial by counting the number of parameters in $m$.
For an HPO problem, we are mainly interested in predicting the parameter value of the next trial given the history as an HPO policy. Therefore, we would focus on learning the conditional distribution of $P(\widehat{x}_t^{(d)}|\widehat{m}, \widehat{h}_{t}^{(d-1)})$. 
%With a properly trained sequence model, we could use it as an HPO policy by sampling parameter $\widehat{\vx}_t = \left[\widehat{x}_{t}^{(1)}, \dots, \widehat{x}_{t}^{(D)}\right]$ sequentially given $(\widehat{m}, \widehat{h}_{t-1})$, and decode the token sequence back to the original search space. 
Moreover, we would also model the conditional distribution of the function value $P(\widehat{y}_t|\widehat{m}, \widehat{h}_{t}^{(D)})$ as a by-product of the training process.

In this paper, we use a T5 Transformer with an encoder-decoder architecture\citep{2020t5}. This model, parameterized by $\theta$, consists of an encoder $E$ and decoder $D$. The encoder takes in an input conditioning sequence, which in our case is the tokenized metadata $\widehat{m}$, and outputs a sequence of embeddings of the same length as the input. The decoder takes in the output of the encoder $E(\widehat{m})$ and an input target sequence, which in our case is the tokenized sequence of the history $\widehat{h}$, and outputs a sequence of token distributions. By applying a causal attention matrix in the decoder, we enforce the Transformer to predict the distribution of the $n$-th token conditioned on the metadata $\widehat{m}$ and $\widehat{h}[1:n-1]$, the historical token sequence up to the $(n-1)$-th token. The entire process can be seen as:
% \begin{equation}
%     \tilde{P}_{\theta}(\widehat{h}_n|\widehat{m}, \widehat{h}_{1:n-1}) = \mathrm{SoftMax} \left[ D_{\theta_D}(E_{\theta_E}(\widehat{m}), \widehat{h}_{1:n-1}) \right]
% \end{equation}
\begin{equation}
    P_{\theta}(\widehat{h}[n]|\widehat{m}, \widehat{h}[1:n-1]) = \mathrm{SoftMax} \left[ D_{\theta_D}(E_{\theta_E}(\widehat{m}), \widehat{h}[1:n-1]) \right]
\end{equation}


==> storage/notes.tex <==
\section{Related Work}

%This can lead to the issue of domain shift, as the structure of cheap tasks used for training (e.g. BBOB functions \citep{} used in \citep{chen2017learning}) may be very different from tasks one ideally wishes to optimize over (e.g. NASBENCH \citep{}).



%TODO(wangzi): rewrite the following.

%End-to-end learning  volpp2020meta is popular meta BO approach for hyperparameter tuning that learns a strategy to suggest new query points based on past history of BO. \citep{volpp2020meta} learns acquisition functions via reinforcement learning.

%multi-task BO~\citep{swersky2013multi, poloczek2017multi, yogatama2014efficient} and transfer learning BO using contextual GPs~\citep{krause2011contextual, bardenet2013collaborative, poloczek2016warm} are both meta BO approaches. Some meta BO methods have also been studied for hyperparamter tuning tasks in machine learning~\citep{feurer2015efficient}.



%Model-based metalearning all utilize the notion of a function regressor, which is able to learn from offline data, providing an advantage over online RNN-based approaches. The most common function regressor used is a Gaussian Process (GP). 

